How Over-Parameterization Slows Down Gradient Descent in Matrix Sensing: The Curses of Symmetry and Initialization

This paper rigorously shows how over-parameterization changes the convergence behaviors of gradient descent (GD) for the matrix sensing problem, where the goal is to recover an unknown low-rank ground-truth matrix from near-isotropic linear measurements. First, we consider the symmetric setting with the symmetric parameterization where $M^* \in \mathbb{R}^{n \times n}$ is a positive semi-definite unknown matrix of rank $r \ll n$, and one uses a symmetric parameterization $XX^\top$ to learn $M^*$. Here $X \in \mathbb{R}^{n \times k}$ with $k > r$ is the factor matrix. We give a novel $\Omega (1/T^2)$ lower bound of randomly initialized GD for the over-parameterized case ($k >r$) where $T$ is the number of iterations. This is in stark contrast to the exact-parameterization scenario ($k=r$) where the convergence rate is $\exp (-\Omega (T))$. Next, we study asymmetric setting where $M^* \in \mathbb{R}^{n_1 \times n_2}$ is the unknown matrix of rank $r \ll \min\{n_1,n_2\}$, and one uses an asymmetric parameterization $FG^\top$ to learn $M^*$ where $F \in \mathbb{R}^{n_1 \times k}$ and $G \in \mathbb{R}^{n_2 \times k}$. Building on prior work, we give a global exact convergence result of randomly initialized GD for the exact-parameterization case ($k=r$) with an $\exp (-\Omega(T))$ rate. Furthermore, we give the first global exact convergence result for the over-parameterization case ($k>r$) with an $\exp(-\Omega(\alpha^2 T))$ rate where $\alpha$ is the initialization scale. This linear convergence result in the over-parameterization case is especially significant because one can apply the asymmetric parameterization to the symmetric setting to speed up from $\Omega (1/T^2)$ to linear convergence. On the other hand, we propose a novel method that only modifies one step of GD and obtains a convergence rate independent of $\alpha$, recovering the rate in the exact-parameterization case.

==> change.tex <==
\subsection{Proof Sketch of Theorem \ref{thm:fast method}}\nuoya{Need to make it more simple}
First, suppose we modify the matrix $\widetilde{F}_{T^{(3)}}, \widetilde{G}_{T^{(3)}}$ to $F_{T^{(3)}}$ and $G_{T^{(3)}}$ at $t =T^{(3)},$ then $\|F_{T^{(3)}}\|^2 = \lambda_{\max}((F_{T^{(3)}})^\top F_{T^{(3)}})=\beta^2$ and $\|U_{T^{(3)}}\|^2 \le \beta^2.$ 
%Hence by $\sigma_1(U)\cdot \sigma_r(V) \ge \sigma_r(UV^\top )$, we can derive $\sigma_r(V_{T^{(3)}})\ge \frac{\sigma_r(U_{T^{(3)}}V_{T^{(3)}}^\top )}{\sigma_1(U_{T^{(3)}})}\ge \sigma_r/2c$, where we use the fact that $\sigma_r(U_{T^{(3)}}V_{T^{(3)}}^\top )=\sigma_r(\widetilde{U}_{T^{(3)}}\widetilde{V}_{T^{(3)}}^\top)\ge \sigma_r-\|\widetilde{U}_{T^{(3)}}\widetilde{V}_{T^{(3)}}^\top -\Sigma\|\ge \sigma_r/2.$ 
Also, by $\|\widetilde{F}_{T^{(3)}}\|\le 2\sqrt{\sigma_1}$, we can get $\|G_{T^{(3)}}\| \le \|\widetilde{G}_{T^{(3)}}\|\cdot \frac{\|\widetilde{F}_{T^{(3)}}\|}{c}\le \|\widetilde{G}_{T^{(3)}}\|\cdot \frac{2\sqrt{\sigma_1}}{c}$ is still bounded. Similarly, $\|V_{T^{(3)}}\|\le \|\widetilde{V}_{T^{(3)}}\|\cdot \frac{2\sqrt{\sigma_1}}{c}$ and $\|K_{T^{(3)}}\| \le \|\widetilde{K}_{T^{(3)}}\| \cdot \frac{2\sqrt{\sigma_1}}{c}$ is still bounded.  With these conditions, define $S_t= \max\{\|U_tK_t^\top \|, \|J_tK_t^\top \|\}$ and $P_t = \max\{\|J_tV_t^\top \|, \|U_tV_t^\top -\Sigma\|\}$, by the updating rule, 
for $\|K_t\|$, since we can prove $\lambda_{\min}(F_t^\top F_t)\ge \beta^2/2$ for all $t \ge T^{(3)}$ using induction, we can write the updating rule as 
\begin{align}
    \|K_{t+1}\|&\le \|K_t\|\|1-\eta F_t^\top F_t\| + 2\delta_{2k+1}\cdot \|F_tG_t^\top -\Sigma\|\max\{\|U_t\|,\|J_t\|\}\\
    &\le \|K_t\|\cdot \left(1-\frac{\eta \beta^2}{2}\right) + \left(4\eta \delta_{2k+1}c\cdot P_t + 4\beta^2\eta \delta_{2k+1}\|K_t\|\right).\label{update rule of Kt main text fast}
\end{align}
The first term of Eq.\ref{update rule of Kt main text fast} ensures the linear convergence, and the second term represents the perturbation term. To control the perturbation term, for $P_t$, we further calculate
(The details are provided in Appendix \ref{appendix: proof of fast})
\begin{align}
    P_{t+1}\le \left(1-\eta\sigma_r^2/8\beta^2\right) P_t + \eta \|K_t\|\cdot \widetilde{\cO}\left(\left(\delta_{2k+1}\sigma_1+\sqrt{\alpha \sigma_1^{7/4}}\right)/c\right).\label{update rule of Pt main}
\end{align}
The last inequality uses the fact that $S_t \le \|K_t\|\cdot \max\{\|U_t\|,\|J_t\|\}\le \|K_t\|\cdot \|F_t\| \le \sqrt{2}c\cdot \|K_t\|.$

% On the other hand, for $\|K_t\|$, since we can prove $\lambda_{\min}(F_t^\top F_t)\ge \beta^2/2$ for all $t \ge T^{(3)}$ using induction, we can write the updating rule as 
% \begin{align}
%     \|K_{t+1}\|&\le \|K_t\|\|1-\eta F_t^\top F_t\| + 2\delta_{2k+1}\cdot \|F_tG_t^\top -\Sigma\|\max\{\|U_t\|,\|J_t\|\}\\
%     &\le \|K_t\|\cdot \left(1-\frac{\eta \beta^2}{2}\right) + \left(4\eta \delta_{2k+1}c\cdot P_t + 4\beta^2\eta \delta_{2k+1}\|K_t\|\right).\label{update rule of Kt main text fast}
% \end{align}
Combining Eq. \eqref{update rule of Pt main} and Eq.\eqref{update rule of Kt main text fast}, we can show that $P_t + \sqrt{\sigma_1}\|K_t\|$ converges at a linear rate $(1-\cO(\eta \beta^2)),$ since the second term of Eq. \eqref{update rule of Pt main} and Eq.\eqref{update rule of Kt main text fast} contain $\delta_{2k+1}$ or $\alpha$, which is relatively small and can be canceled by the first term. Hence $\|F_tG_t^\top -\Sigma\| \le 2P_t + 2S_t \le 2P_t + \sqrt{2}c\|K_t\|$ converges at a linear rate. 


\subsection{Proof of Theorem \ref{thm:fast method}}
\label{sec: proof.fast_method}
At time $t\ge T^{(3)}$, we have $\sigma_{\min}(U_{T^{(3)}}V_{T^{(3)}}) \ge \sigma_{\min}(\Sigma) - \| U_{T^{(3)}}V_{T^{(3)}}^\top  - \Sigma\| \ge \sigma_r-\alpha^{1/2}\cdot \sigma_1^{3/4} \ge \sigma_r/2. $ The last inequality holds because $\alpha = O(\kappa^{-3/2}\cdot \sqrt{\sigma_r})$. 
Then given that $\|F_{T^{(3)}}\|^2 = \lambda_{\max}((F_{T^{(3)}})^\top F_{T^{(3)}}) = \beta^2 $, we have $\|U_{T^{(3)}}\|^2 \le \beta^2$. Hence by $\sigma_1(U) \cdot \sigma_r(V) \ge \sigma_r(UV^\top )$, we have $$\sigma_r(V_{T^{(3)}}) \ge \frac{\sigma_r(U_{T^{(3)}}V_{T^{(3)}})}{\sigma_1(U_{T^{(3)}})}\ge \frac{\sigma_r}{2c}.$$

Also, by $\sigma_1'=\|\widetilde{F}_{T^{(3)}}\|\le 2\sqrt{\sigma_1},$ we can get $$\|G_{T^{(3)}}\| \le \|\widetilde{G}_{T^{(3)}}\|\|B\Sigma_{inv}^{-1}\| \le \|\widetilde{G}_{T^{(3)}}\| \cdot \frac{\sigma_1'}{c}\le\|\widetilde{G}_{T^{(3)}}\| \cdot \frac{2\sqrt{\sigma_1}}{c}.$$ Similarly, $\|V_{T^{(3)}}\| \le  \|\widetilde{V}_{T^{(3)}}\| \cdot \frac{2\sqrt{\sigma_1}}{c}$ and $\|K_{T^{(3)}}\| \le  \|\widetilde{K}_{T^{(3)}}\| \cdot \frac{2\sqrt{\sigma_1}}{c}$.

Denote $S_t = \max\{\|U_tK_t^\top \|, \|J_tK_t^\top \|\}, P_t = \max\{\|J_tV_t^\top \|, \|U_tV_t^\top -\Sigma\|\}$. Now we prove the following statements by induction:
\begin{gather}
    P_{t+1} \le \left(1-\frac{\eta\sigma_r^2}{8\beta^2}\right)P_t + \eta S_t \cdot \cO \left(\frac{\log(\sqrt{\sigma_1}/n\alpha)\delta_{2k+1}\kappa^2 \sigma_1^2+\sqrt{\alpha}\sigma_1^{7/4}}{\beta^2}\right)\label{fast: condition 2}\\
    \|F_{t+1}G_{t+1}^\top -\Sigma\| \le \frac{c^6}{\sigma_1^2}\left(1-\frac{\eta \beta^2}{2}\right)^{t+1-T^{(3)}}\le \sigma_r/2\label{fast: condition 3}\\
    \max\{\|F_{t+1}\|,\|G_{t+1}\|\} \le 4 \sigma_1/c \label{fast: condition 1}
    \\ \frac{\beta^2}{2} I \le F_{t+1}^\top F_{t+1} \le 2\beta^2 I \label{fast: condition 4}\\
    \|K_{t}\|\le \cO(2\sqrt{\alpha}\sigma_1^{1/4}+\delta_{2k+1}\log(\sqrt{\sigma_1}/n\alpha)\cdot \kappa^2\sqrt{\sigma_1}) \cdot \frac{2\sqrt{\sigma_1}}{c} \label{fast: condition 5}
\end{gather}

%Now we first assume $\max\{\|F_t\|,\|G_t\|\} \le 4\sqrt{\sigma_1}\cdot \sigma_1/c $, and we will prove it later.
\paragraph{Proof of Eq.\eqref{fast: condition 2}}

First, since $\|F_t\|^2 = \lambda_{\max}((F_t)^\top F_t) \le 2\beta^2 $, we have $\|U_{t}\|^2 \le 2\beta^2$. Then because  $\sigma_{\min}(U_tV_t)\ge \sigma_{\min}(\Sigma) - \|U_tV_t^\top -\Sigma\| \ge \sigma_r/2$, by $\sigma_1(U) \cdot \sigma_r(V) \ge \sigma_r(UV^\top )$, we have $$\sigma_r(V_{t}) \ge \frac{\sigma_r(U_{t}V_{t})}{\sigma_1(U_{t})}\ge \frac{\sigma_r}{2c}.$$



we write down the updating rule as 
\begin{align*}
    &\quad U_{t+1}V_{t+1}^\top -\Sigma %\\&= U_tV_t^\top -\Sigma -\eta U_tU_t^\top (U_tV_t^\top -\Sigma) - \eta (U_tV_t^\top -\Sigma) V_tV_t^\top  - \eta U_tK_t^\top K_tV_t^\top -\eta U_tJ_t^\top J_tV_t^\top   + A\\
    \\&= (1-\eta U_tU_t^\top )(U_tV_t^\top -\Sigma)(1-\eta V_tV_t^\top )  -\eta U_tK_t^\top K_tV_t^\top -\eta U_tJ_t^\top J_tV_t^\top  + B_t
\end{align*}
where $B_t$ contains the $\cO(\eta^2)$ terms and $\cO(E_i(F_tG_t^\top -\Sigma))$ terms 
\begin{align*}
    \|B_t\| &\le 4\eta \delta_{2k+1} (F_tG_t^\top -\Sigma) \max\{\|F_t\|^2,\|G_t\|^2\} + \cO(\eta^2\|F_tG_t^\top -\Sigma\|^2 \max\{\|F_t\|^2,\|G_t\|^2\}) 
\end{align*}
Hence we have 
\begin{align}
    &\quad \|U_{t+1}V_{t+1}^\top -\Sigma\| \\&\le (1-\frac{\eta\sigma_r^2}{4\beta^2})\|U_tV_t^\top -\Sigma\| + \eta \|U_tK_t^\top \|\|K_tV_t^\top \| + \eta \|J_tV_t^\top \|\|J_t^\top U_t^\top \| + \|B_t\|\\&\le (1-\frac{\eta\sigma_r^2}{4\beta^2})P_t + \eta S_t \|K_t\| \|V_t\| + \eta P_t \| J_t\|\|U_t\| + \|B_t\|\\&\le (1-\frac{\eta\sigma_r^2}{4\beta^2})P_t + \eta S_t \cdot \frac{4\sigma_1}{\beta^2}\cdot \cO\left(2\sqrt{\alpha}\sigma_1^{1/4}+\delta_{2k+1}\log(\sqrt{\sigma_1}/n\alpha)\cdot \kappa^2\sqrt{\sigma_1}\right)\cdot 2\sqrt{\sigma_1} + \eta P_t c\cdot c \\&\qquad   + 4\eta \delta_{2k+1}\cdot 2(P_t+S_t)\cdot 4\sigma_1\cdot \frac{4\sigma_1}{\beta^2} + \cO(\eta^2(P_t+S_t)^2\cdot 4\sigma_1\cdot \frac{4\sigma_1}{\beta^2})\\
    &\le  \left(1-\frac{\eta\sigma_r^2}{8\beta^2}\right)P_t + \eta S_t \cdot \cO \left(\frac{\log(\sqrt{\sigma_1}/n\alpha)\delta_{2k+1}\kappa^2 \sigma_1^2+\sqrt{\alpha}\sigma_1^{7/4}}{\beta^2}\right)\label{ineq: PtSt recursion}
\end{align}
The last inequality uses the fact that 
\begin{gather}
    \beta^2 = \cO(\sigma_r^{1/2})\\
    \delta_{2k+1} = \cO(\kappa^{-2})\\
    P_t + S_t \le 2\|F_tG_t^\top -\Sigma\| \le \cO(\sigma_1^2/\beta^2)\le 1/\eta.
\end{gather}
% which means that 
% \begin{gather}
%     c^3 \le \frac{\sigma_r}{8}\label{ineq: upper bound of c 2}\\
%     c  \ge \frac{8\sigma_1^2 \delta_{2k+1}}{\sigma_r}\label{ineq: lower bound of c}\\
%     \eta \le \frac{\sigma_r}{32\sigma_1^3 c^3}\label{ineq: upper bound of eta}
% \end{gather}
Similarly, we have 
\begin{align*}
    &\quad \|J_{t+1}V_{t+1}^\top \|\\&\le \left(1-\eta J^\top J\right) JV^\top  (1-\eta V^\top V) -\eta JK^\top KV^\top  - \eta JU^\top (UV^\top -\Sigma) +C_t  
\end{align*}
where $C_t$ satisfies that 
\begin{align*}
    \|C_t\| &\le 4\eta \delta_{2k+1} (F_tG_t^\top -\Sigma)\max\{\|F_t\|^2, \|G_t\|^2\}  + \cO(\eta^2\|F_tG_t^\top -\Sigma\|\max\{\|F_t\|^2, \|G_t\|^2\}) \\
    &\le 4\eta \delta_{2k+1}\cdot 2(P_t+S_t)\cdot \frac{16\sigma_1^2}{\beta^2} + \cO(\eta^2(P_t+S_t)\cdot \sigma_1\cdot \frac{\sigma_1}{\beta^2}).%\\&= \frac{4\eta \delta_{2k+1}\sigma_1^2\cdot (P_t+S_t)}{\beta^2} + \cO(\frac{4\eta^2\sigma_1^3}{\beta^2} (P_t+S_t)).
\end{align*}

Thus similar to Eq.\eqref{ineq: PtSt recursion}, we have 
\begin{align*}
    \|J_{t+1}V_{t+1}^\top  \| 
    \le \left(1-\frac{\eta\sigma_r^2}{8\beta^2}\right)P_t + \eta S_t \cdot \cO \left(\frac{\log(\sqrt{\sigma_1}/n\alpha)\delta_{2k+1}\kappa^2 \sigma_1^2+\sqrt{\alpha}\sigma_1^{7/4}}{\beta^2}\right).
\end{align*}
Hence we have 
\begin{align*}
    P_{t+1} \le \left(1-\frac{\eta\sigma_r^2}{8\beta^2}\right)P_t + \eta S_t \cdot \cO \left(\frac{\log(\sqrt{\sigma_1}/n\alpha)\delta_{2k+1}\kappa^2 \sigma_1^2+\sqrt{\alpha}\sigma_1^{7/4}}{\beta^2}\right).
\end{align*}
\paragraph{Proof of Eq.\eqref{fast: condition 3}}

We have
$S_t \le \|K_t\| \cdot \max\{\|U_t\|, \|J_t\|\}\le \|K_t\| \cdot \|F_t\|\le \sqrt{2}c\cdot \|K_t\|$. So the inequality above can be rewritten as 
\begin{align}
    P_{t+1} &\le \left(1-\frac{\eta\sigma_r^2}{8\beta^2}\right)P_t + \eta  \sqrt{2}c \cdot\|K_t\|\cdot  \cO \left(\frac{\log(\sqrt{\sigma_1}/n\alpha)\delta_{2k+1}\kappa^2 \sigma_1^2+\sqrt{\alpha}\sigma_1^{7/4}}{\beta^2}\right) \\&= \left(1-\frac{\eta\sigma_r^2}{8\beta^2}\right)P_t + \eta \|K_t\| \cdot \cO \left(\frac{\log(\sqrt{\sigma_1}/n\alpha)\delta_{2k+1}\kappa^2 \sigma_1^2+\sqrt{\alpha}\sigma_1^{7/4}}{c}\right)
\end{align}
Also, for $K_{t+1}$, we have 
\begin{align}
    \|K_{t+1}\| &= \|K_t\|\|(1-\eta F_t^\top F_t)\| + 2\delta_{2k+1}\cdot \|F_tG_t^\top -\Sigma\|\max\{\|U_t\|, \|J_t\|\}\\
    &\le \|K_t\|(1-\frac{\eta \beta^2}{2}) + 2\eta \delta_{2k+1}\cdot (P_t+S_t)\cdot \sqrt{2}c \\
    &\le \|K_t\|(1-\frac{\eta \beta^2}{2}) +2\eta \delta_{2k+1}\cdot P_t\cdot \sqrt{2}c  + 2\eta \delta_{2k+1}\cdot \sqrt{2}c  \|K_t\| \cdot\sqrt{2}c  \\
    &=\|K_t\|(1-\frac{\eta \beta^2}{2}) +4\eta \delta_{2k+1}\cdot c P_t  + 4\beta^2\eta \delta_{2k+1}\cdot  \|K_t\|
\end{align}
Thus we can get 
\begin{align}
   &\quad  P_{t+1} + \sqrt{\sigma_1}\|K_{t+1}\| \\&\le \max\{1-\frac{\eta\sigma_r^2}{8\beta^2}, 1-\frac{\eta \beta^2}{2}\}(P_t + \|K_t\|)  \\&\qquad +\eta\max\left\{\cO \left(\frac{\log(\sqrt{\sigma_1}/n\alpha)\delta_{2k+1}\kappa^2 \sigma_1^{3/2}+\sqrt{\alpha}\sigma_1^{5/4}}{c}\right)+ 4\beta^2 \delta_{2k+1}, 4c \sqrt{\sigma_1}\delta_{2k+1}\right\}\cdot (P_t + \sqrt{\sigma_1}\|K_t\|)\\
    &\le (1-\frac{\eta \beta^2}{4})(P_t + \sqrt{\sigma_1}\|K_t\|).
\end{align}
The last inequality uses the fact that $c\le \cO(\sigma_r^{1/2})$ and 
\begin{align}
\delta_{2k+1} \le \cO(c/\sqrt{\sigma_1}\log(\sqrt{\sigma_1}/n\alpha)).
\end{align}
Hence \begin{align}
    \|K_{t}\| &\le (P_{T^{(3)}}/\sqrt{\sigma_1}+\|K_{T^{(3)}}\|)\cdot \left(1-\frac{\eta \beta^2}{2}\right)^{t-T^{(3)}}\\
    &\le \|K_{T^{(3)}}\|+\|F_tG_t^\top -\Sigma\|/\sqrt{\sigma_1}\\
    &\le \cO(\sqrt{\alpha}\sigma_1^{1/4}+\delta_{2k+1}\log(\sqrt{\sigma_1}/n\alpha)\cdot \kappa^2\sqrt{\sigma_1})+\alpha^{1/2}\cdot \sigma_1^{1/4}\\
    &= \cO(\sqrt{\alpha}\sigma_1^{1/4}+\delta_{2k+1}\log(\sqrt{\sigma_1}/n\alpha)\cdot \kappa^2\sqrt{\sigma_1})
\end{align}
% which holds by $c \le 1$ and   
% \begin{align}
%     c \ge \max\left\{(16\delta_{2k+1})^{2/5}, \widetilde{\cO}\left(\frac{\delta_{2k+1}^{1/7}\sigma_1^2)}{\sigma_r}\right)\right\}\ge \max\left\{(16\delta_{2k+1})^{2/5}, \widetilde{\cO}\left(\left(\frac{\delta_{2k+1}\sigma_1^4)}{\sigma_r}\right)^{2/7}\right)\right\}.\label{ineq:lower bound of c 2}
% \end{align}
Hence $P_t + \sqrt{\sigma_1}\|K_t\|$ is linear convergence. Hence by $c\le \sqrt{\sigma_1}$, \begin{align}\quad \|F_{t+1}G_{t+1}^\top -\Sigma\|& \le 2P_{t+1} + 2S_{t+1} \\&\le 2P_{t+1} + \sqrt{2}c\|K_{t+1}\|\\&\le (2+\sqrt{2}c/\sqrt{\sigma_1})(P_{t+1} + \sqrt{\sigma_1}\|K_{t+1}\|)\\&\le 4(P_{T^{(3)}} + \sqrt{\sigma_1}\|K_{T^{(3)}}\|)\cdot  \left(1-\frac{\eta \beta^2}{2}\right)^{t+1-T^{(3)}}\end{align}
% Last, by $c\ge 4\sigma_1\alpha^{1/24},$ and
% \begin{align*}
%     c\ge \cO(\delta_{2k+1}^{1/7}\cdot \sigma_1^2/\sigma_r)\ge \left(\widetilde{\cO}(2\sigma_1^2 \delta_{2k+1} \cdot \sigma_1^{3/2}/\sigma_r)\right)^{1/7} = \widetilde{\cO}(\delta_{2k+1}^{1/7}\cdot \sigma_1^{7/14}/\sigma_r^{1/7})
% \end{align*}
Last, 
note that by $c\ge \cO(\alpha^{1/6}\sigma_1^{5/12})$ and $\delta_{2k+1}\le \cO(c^4/\kappa\sigma_1^{2}\log(\sqrt{\sigma_1}/n\alpha))$ $$P_{T^{(3)}} + \sqrt{\sigma_1}\|K_{T^{(3)}}\| \le \alpha^{1/2}\cdot \sigma_1^{3/4} + \sqrt{\sigma_1}\cdot\cO(\log(\sqrt{\sigma_1}/n\sqrt{\alpha})\delta_{2k+1}\cdot \sigma_1^{3/2}/\sigma_r) \cdot (2\sqrt{\sigma_1}/c)\le c^6/\sigma_1^2$$
we have 
\begin{align}
    \|F_{t+1}G_{t+1}^\top -\Sigma\| \le \frac{c^6}{\sigma_1^2} \left(1-\frac{\eta \beta^2}{2}\right)^{t+1-T^{(3)}}
\end{align}
\paragraph{Proof of Eq.\eqref{fast: condition 1}}

Suppose $\max\{\|F_{t'}\|,\|G_{t'}\|\} \le 4\sqrt{\sigma_1}\cdot \sqrt{\sigma_1}/c = 4\sigma_1/c$ for all $t' \in [T^{(3)}, t]$, 
then the changement of $F_{t+1}$ and $G_{t+1}$ can be bounded by 
\begin{align*}
    \|F_{t+1}-F_{T^{(3)}}\| &\le\eta  \sum_{t'=T^{(3)}}^{t}2\| F_{t'}G_{t'}-\Sigma\|\|G_{t'}\|\le \eta\cdot 2\cdot \frac{c^6}{\sigma_1^2}\cdot \frac{2}{\eta \beta^2}\frac{4\sigma_1}{c} =\frac{16c^3}{\sigma_1}\\
    \|G_t-G_{T^{(3)}}\| &\le \eta\sum_{t'=T^{(3)}}^{t-1}2\| F_{t'}G_{t'}-\Sigma\|\|F_{t'}\|\le \frac{16c^3}{\sigma_1}
\end{align*}

Then by the fact that $c\le \cO(\sigma_1^{-1/2})$, we can show that 
\begin{gather*}
    \|F_{t+1}\| \le \|F_{T^{(3)}}\| + \|F_{t+1}-F_{T^{(3)}}\| \le \frac{2\sigma_1}{c} + \frac{16c^3}{\sigma_1}\le \frac{4\sigma_1}{c},\\
    \|G_{t+1}\| \le \|G_{T^{(3)}}\| + \|G_{t+1}-G_{T^{(3)}}\| \le \frac{2\sigma_1}{c} + \frac{16c^3}{\sigma_1}\le \frac{4\sigma_1}{c}.
\end{gather*}
\paragraph{Proof of Eq.\eqref{fast: condition 4}}

Moreover, we have 
\begin{align*}
    \sigma_{k}(F_{t+1}) &\ge \sigma_{k}(F_{T^{(3)}})-\sigma_{\max}(F_{t+1}-F_{T^{(3)}})\\&=\sigma_{k}(F_{T^{(3)}})-\|F_{t+1}-F_{T^{(3)}}\| \\&\ge c - \frac{16c^3}{\sigma_1}\\
    &\ge c/\sqrt{2},
\end{align*}
and 
\begin{align*}
    \|F_t\| \le \|F_{T^{(3)}}\| + \|F_t-F_{T^{(3)}}\|\le c +\frac{16c^3}{\sigma_1} \le \sqrt{2}c.
\end{align*}
The last inequality is because $c \le \cO(\sigma_1^{-1/2})$.
Hence since $F_{t+1} \in \RR^{n\times k}$, we have 
\begin{align}
    \frac{\beta^2}{2}I\le F_{t+1}^\top F_{t+1}\le 2\beta^2I
\end{align}
Thus, we complete the proof.




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
%\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

